XLEnt: Mining a Large Cross-lingual Entity Dataset with Lexical-Semantic-Phonetic Word Alignment

Cross-lingual named-entity lexica are an important resource to multilingual NLP tasks such as machine translation and cross-lingual wikification. While knowledge bases contain a large number of entities in high-resource languages such as English and French, corresponding entities for lower-resource languages are often missing. To address this, we propose Lexical-Semantic-Phonetic Align (LSP-Align), a technique to automatically mine cross-lingual entity lexica from mined web data. We demonstrate LSP-Align outperforms baselines at extracting cross-lingual entity pairs and mine 164 million entity pairs from 120 different languages aligned with English. We release these cross-lingual entity pairs along with the massively multilingual tagged named entity corpus as a resource to the NLP community.

==> 02related.tex <==
\section{Related Work}

Our work is most closely related to efforts in annotation projection based on word alignment results. In work by~\citep{kim2010cross}, heuristic approaches along with alignment correction using an alignment dictionary of entity mentions was used to project annotations. \citep{das2011unsupervised} introduce a novel label propagation technique that creates a tag lexicon for the target language; this serves to smooth the projected labels. \citep{wang2014cross} follow a similar projection scheme but instead project model expectation rather than labels allowing for the transfer of word boundary uncertainty. Additional work jointly performs word alignment while training bilingual name tagging~\cite{wang2013joint}. However this method assumes the availability of named entity taggers in both languages, and both taggers need to have comparable and diverse strengths to improve and learn from each other. This poses a problem for low-resource language for which many have no high-quality named entity taggers.

Other methods have leveraged bilingual embeddings for projection. One of these methods develop heuristic schemes that effectively selects high-quality projection-labeled data from noisy
data and trains named entity detectors~\cite{ni2017weakly}. The same work also proposes projecting distributed representations of words (word embeddings) from a target language to
a source language, so that the source language NER system can be applied to the target language without re-training. However, since languages may show different linguistic properties, it's difficult to align embedding spaces from different languages perfectly. Further work proposes techniques identifying named entity translations using bilingual word embeddings where self-attention allows for a degree of flexibility with respect to word order~\cite{xie2018neural}.




\todo{ Few other pointers to cross lingual projection (see source)
Semantic role (2009)
%https://arxiv.org/pdf/1401.5694.pdf

Weakly Supervised Cross-Lingual Named Entity  (2017)
%https://www.aclweb.org/anthology/P17-1135.pdf

Entity Projection (2019)
%https://www.aclweb.org/anthology/D19-1100v2.pdf

Data Transfer with Unlabeled data (2020)
%https://arxiv.org/pdf/2007.07683.pdf

Others
%Examples include parts of
%speech (Yarowsky et al., 2001; Hi & Hwa, 2005), chunks (Yarowsky et al., 2001), dependencies (Hwa et al., 2002), word senses (Diab & Resnik, 2002; Bentivogli & Pianta, 2005),
%information extraction markup (Riloff, Schafer, & Yarowsky, 2002), coreference chains (Postolache, Cristea, & Orasan, 2006), temporal information (Spreyer & Frank, 2008), and LFG
%f-structures (Tokarczyk & Frank, 2009).
}

Word alignment models have been a tool for projecting annotation labels to other languages.
\todo{add literature for word alignment}




Phonetic signals have often been used for entity detection. 
\todo{Add literature for transliteration}


Dense word and text representations have been widely investigated for a variety of NLP tasks. To address the effect of word-sparsity, embedding techniques have been proposed that leverage subwords to enrich word embeddings~\cite{bojanowski2017enriching}. These embeddings rely on the finer-granularity of subwords to construct semantically meaningful representations even when the individual words themselves are infrequent. To bring the benefiit of word representations to cross-lingual NLP, many approaches have successfully jointly embedded text in different languages into the same semantic space. For such cases, word and its translation are close in the embedding space. Many of these approaches have leveraged some supervision to train bi-lingual embeddings~\cite{espana2017empirical,yang2019improving}. Other methods have introduced full-unsupervised techniques  to jointly align two embeddings spaces~\cite{lample2018unsupervised}. However, training bilingual embedding models for each language pair is difficult to scale beyond a handful of language pairs. To address this, techniques that jointly embed 93 languages in the same space have been proposed~\cite{artetxe2019massively}.


While most applications to cross-lingual tag projections are applied to gold-standard parallel sentences, this data is often limited. As such, to ensure a broad collection of domains and diversity of named entities and terminology, we mine entities from large web-based comparable corpora. There has been a recent surge in interest in mining the web for comparable corpora~\cite{el2020searching}. Such methods first crawl multilingual web domains likely to contain parallel texts~\cite{banon2020paracrawl}, then perform document alignment to identify potentially comparable documents~\cite{el2020massively} and mine bitexts. These techniques and others have been used to mine parallel data from Wikipedia~\cite{schwenk2019wikimatrix} as well as Common Crawl~\cite{el2020massive,schwenk2019ccmatrix}.

==> 06casestudy.tex <==
% \section{Qualitative Analysis}
% In addition to quantitative entity translation and machine translation experiments, we also perform a human-led qualitative analysis. Under this scheme, we attempt to identify what scenarios lead to better named entity extraction for our three signals and whether our combined approach leverages the best signal for each entity matching.

% As entity pairs for which our three signals completely agree are less interesting, we first select entity pairs for which our three signals suggest different target entities with one selecting a high fuzzy-F1 entity. 


